High Order Semi-implicit WENO Schemes for All Mach Full Euler System of Gas Dynamics

In this paper, we propose a new high order semi-implicit scheme for the all Mach full Euler equations of gas dynamics. Material waves are treated explicitly, while acoustic waves are treated implicitly, thus avoiding severe CFL restrictions for low Mach flows. High order accuracy in time is obtained by semi-implicit temporal integrator based on the IMEX Runge-Kutta (IMEX-RK) framework. High order in space is achieved by finite difference WENO schemes with characteristic-wise reconstructions adapted to the semi-implicit IMEX-RK time discretization. Type A IMEX schemes are constructed to handle not well-prepared initial conditions. Besides, these schemes are proven to be asymptotic preserving and asymptotically accurate as the Mach number vanishes for well-prepared initial conditions. Divergence-free property of the time-discrete schemes is proved. The proposed scheme can also well capture discontinuous solutions in the compressible regime, especially for two dimensional Riemann problems. Numerical tests in one and two space dimensions will illustrate the effectiveness of the proposed schemes.

==> mainshared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{algorithmic}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{claim}{Claim}

% Sets running headers as well as PDF title and authors
%\headers{An Example Article}{D. Doe, P. T. Frank, and J. E. Smith}
%
%% Title. If the supplement option is on, then "Supplementary Material"
%% is automatically inserted before the title.
%\title{An Example Article\thanks{Submitted to the editors DATE.
%\funding{This work was funded by the Fog Research Institute under contract no.~FRI-454.}}}
%
%% Authors: full names plus addresses.
%\author{Dianne Doe\thanks{Imagination Corp., Chicago, IL
%  (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
%\and Paul T. Frank\thanks{Department of Applied Mathematics, Fictional University, Boise, ID
%  (\email{ptfrank@fictional.edu}, \email{jesmith@fictional.edu}).}
%\and Jane E. Smith\footnotemark[3]}

\usepackage{amsopn}
\DeclareMathOperator{\diag}{diag}


%%% Local Variables:
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End:


==> packages.tex <==


\theoremstyle{plain}
%\newtheorem{thm}{Theorem}[section]


\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\theoremstyle{plainNoItalics}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{defn}[thm]{Definition}
\newtheorem{rem}[thm]{Remark}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{exa}[thm]{Example}

\newcommand{\f}{\frac}
\newcommand{\ra}{\rightarrow}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\bedef}{\begin{defn}}
\newcommand{\edefn}{\end{defn}}
\newcommand{\bpro}{\begin{prop}}
\newcommand{\epro}{\end{prop}}
\newcommand{\kv}{^{[k]}}
\newcommand{\kvp}{^{[k+1]}}
\newcommand{\kvm}{^{[k-1]}}
\newcommand{\kf}{^{(k)}}
\newcommand{\kfp}{^{(k+1)}}
\newcommand{\kfm}{^{(k-1)}}
%\newcommand{\eps}{\epsilon}
\newcommand{\eps}{\varepsilon}
\newcommand{\nth}{^{th}}
\newcommand{\be}{{\bf e}}
\newcommand{\bq}{{\bf q}}
\newcommand{\bu}{{\bf u}}
\newcommand{\ba}{{\bf a}}
\newcommand{\bx}{{\bf x}}
\newcommand{\bdq}{{\bf \delta q}}
\newcommand{\Dt}{{\Delta t}}
\newcommand{\R}{{\mathbb{R}}}
\newcommand{\Hf}{{\mathcal{H}}}
\newcommand{\Dx}{{\Delta x}}
\newcommand{\Dy}{{\Delta y}}
\newcommand{\ds}{\displaystyle}
\newcommand{\un}{\underline}
\newcommand{\C}{\mathbb{C}}
\newcommand{\rhoe}{_{\varepsilon}}
\newcommand{\comp}[2]{\stackrel{#2}{#1}{}}

\newcommand{\marg}[1]{\marginpar{\tiny{\framebox{\parbox{1.7cm}{#1}}}}}

\newcommand{\he}{\multicolumn} %% He2bing4lie4

\def\Box{\mbox{ }\rule[0pt]{1.5ex}{1.5ex}}

\newcommand\QQ[1]{\textcolor{blue}{#1}}
\newcommand\SB[1]{\textcolor{red}{#1}}


